Point Cloud Generation with Continuous Conditioning

Generative models can be used to synthesize 3D objects of high quality and diversity. However, there is typically no control over the properties of the generated object.This paper proposes a novel generative adversarial network (GAN) setup that generates 3D point cloud shapes conditioned on a continuous parameter. In an exemplary application, we use this to guide the generative process to create a 3D object with a custom-fit shape. We formulate this generation process in a multi-task setting by using the concept of auxiliary classifier GANs. Further, we propose to sample the generator label input for training from a kernel density estimation (KDE) of the dataset. Our ablations show that this leads to significant performance increase in regions with few samples. Extensive quantitative and qualitative experiments show that we gain explicit control over the object dimensions while maintaining good generation quality and diversity.

==> figures/interpolation_height_width.tex <==
\begin{figure}
	\centering

	{\footnotesize
	\begin{tabularx}{\linewidth}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
		& \underline{0.2} & 0.4 & 0.6 & 0.8 & \underline{1.0} & \underline{1.2} \\
		\midrule
		\rotatebox{90}{height} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.20_0.50}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.40_0.50}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.60_0.50}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_0.50}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_1.00_0.50}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_1.20_0.50}.png} \\
		\midrule
		\rotatebox{90}{width} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_0.20}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_0.40}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_0.60}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_0.80}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_1.00}.png} &
		\includegraphics[width=0.16\linewidth]{{graphics/z_1_y_0.50_0.80_1.20}.png} \\
	\end{tabularx}
	}

	\caption{
		\textbf{Sliding over object dimensions}:
		Our method enables direct object dimension manipulation.
		The top shows examples for varying object height and the bottom for varying width.
		The latent vector~$z$ is the same for all depicted objects.
		The columns with the underlined values are from outside the distribution.
	}
	\label{fig:dimension_interpolation_height}
\end{figure}


==> imports/authors.tex <==
\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

